Testing Coverage Functions

A coverage function f over a ground set [m] is associated with a universe U of weighted elements and m subsets A_1,..., A_m of U, and for any subset T of [m], f(T) is defined as the total weight of the elements in the union $\cup_{j\in T} A_j$. Coverage functions are an important special case of submodular functions, and arise in many applications, for instance as a class of utility functions of agents in combinatorial auctions. Set functions such as coverage functions often lack succinct representations, and in algorithmic applications, an access to a value oracle is assumed. In this paper, we ask whether one can test if a given oracle is that of a coverage function or not. We demonstrate an algorithm which makes O(m|U|) queries to an oracle of a coverage function and completely reconstructs it. This gives a polytime tester for succinct coverage functions for which |U$ is polynomially bounded in m. In contrast, we demonstrate a set function which is "far" from coverage, but requires 2^{\tilde{\Theta}(m)} queries to distinguish it from the class of coverage functions.

==> conclusion.tex <==
\section{Concluding Remarks}
In this work we studied the problem of testing coverage functions. Using the $W$-transform we provided a certificate for coverageness, which motivated the notion of the $W$-distance. We gave a reconstruction algorithm which runs in polynomial time for succinct coverage functions, and we exhibited exponential lower bounds on the size of a certificate for non-coverage functions. The latter construction also implies impossibility of distinguishing coverage functions from those with large $W$-distance. Finally, assuming a conjecture, we also showed our construction implies impossibility of  testing 
under the usual notion of distance.
%
%
%In this work, we looked at testing coverage functions. We gave a polytime reconstruction algorithm for succinct coverage functions, and gave lower bounds for distinguishing coverage functions from those with large $W$-distance. We claim that our candidate function $f^*$ also has a large distance in the usual notion and make a reasonable conjecture which would prove this claim. Proving the conjecture is an obvious open question, and we believe a disproof will also be very interesting. Another point regarding $f^*$ is that it needs $N$ to be quite large; it would be nice to obtain a function of polynomial size for the lower bound. We leave this as an open question.

%The main open question in our opinion is that of testing submodular functions. 
%
%Coverage functions possess a lot of structure which we exploited to obtain our results; one probably needs to understand more deeply what property of submodularity can be exploited to either get an upper bound or lower bound. Nevertheless, given our lower bound result, we are more inclined to believe that testing submodular functions might be hard.
%Another avenue to explore is whether there is a different notion of distance for general submodular functions (as there was in the case of coverage functions.) Exploring this might be of independent interest, and might give insights into the question at hand.



Finally, motivated by our reconstruction algorithm for succinct coverage functions, one can ask if there are other succinct submodular functions which can be reconstructed given a value oracle. 
For instance it is known
that rank functions of graphic matroids can be reconstructed using
polynomially many queries (see, for instance, \cite{Tutte},\cite{Seymour}), and so can rank functions of matroids representable over certain fields ($\mathbb{GF}_2,\mathbb{GF}_3$, see \cite{CH96}). Are there other examples which lead to reconstruction algorithms?
%Is there a natural example which cannot be reconstructed?  %\newpage



